Dynamic smooth compressed quadtrees (Fullversion)

We introduce dynamic smooth (a.k.a. balanced) compressed quadtrees with worst-case constant time updates in constant dimensions. We distinguish two versions of the problem. First, we show that quadtrees as a space-division data structure can be made smooth and dynamic subject to split and merge operations on the quadtree cells. Second, we show that quadtrees used to store a set of points in $\mathbb{R}^d$ can be made smooth and dynamic subject to insertions and deletions of points. The second version uses the first but must additionally deal with compression and alignment of quadtree components. In both cases our updates take $2^{\mathcal{O}(d\log d )}$ time, except for the point location part in the second version which has a lower bound of $\Theta (\log n)$---but if a pointer (finger) to the correct quadtree cell is given, the rest of the updates take worst-case constant time. Our result implies that several classic and recent results (ranging from ray tracing to planar point location) in computational geometry which use quadtrees can deal with arbitrary point sets on a real RAM pointer machine.

==> Alignment2.tex <==
\section{Decompressing compressed links in $O(m)$ time instead of $O(mlogm)$ time.} 

Let $A_1$ be a subtree of $T_1$ with as its root a cell $R$ with a compressed leaf $C_a$ as its ancestor. Let $A_1$ store a pointset $P$ with $m$ points. In the previous section assumed that for each $A_1$, its root $R$ was aligned with $C_a$. However, finding a correctly aligned position of a root $R$ of a new uncompressed component $A_1$ when it is inserted by the procedure insertCompressed is not supported in constant time in Real RAM model of computation. The reason is that the length of the compressed link and thus the number of divisions necessary to compute the correctly aligned box for the compressed component, may be arbitrary.\footnote{unless we can use the floor operation (or a different non-standard operation [39, Chapter 2])} Instead of performing this costly computation at the insertion of each new compressed component we instead allow compressed nodes to be associated with any hypercube of an appropriate size that is contained in the compressed ancestor $C_a$. This is a standard way to avoid the above problem~\cite{BLMM11,H11,LM12}. \elena[todo]{check for more links}  \\


In our dynamic quadtree, after a number of split/merge operations on $C_a$ or a number of decompression operations on $A_1$, the size difference between a root $R$ and its ancestor $C_a$ may become less than a factor $\alpha$, in which case we are supposed to \textbf{decompress} the compressed link, replacing it with quadtree cells. 


\begin{figure}[h]
	\centering
	\includegraphics[width=300px]{Pictures/replacementexample.PNG}
    \label{fig:replacementexample}
\end{figure}


We cannot perform this operation if $R$ and $C_a$ are not aligned. Observe that if we need to decompress a link, we can compute the correct root $S$ for $A_1$ in $\mathcal{O}(\alpha)$ time. Moreover, since $R$ was a "good guess"  $|R| = \theta(1)|S|$ and  $P \subset R \cap S $. All that remains is rebuilding $A_1$ on top of $S$. We denote the desired quadtree as $B_1$ and it should store $P$.\\

Figure \ref{fig:replacementexample} shows that $B_1$ and $A_1$ can be completely different quadtrees even though $R$ and $S$ are similar. Building $B_1$ from start will take $\mathcal{O}(m\log(m))$ \textbf{split} and \textbf{insertcompressed} operations. \textbf{The goal of this section is to} use the information from $A_1$ to build $B_1$ in $\mathcal{O}(m)$ \textbf{split} and \textbf{insertcompressed}. Meanwhile we maintain $B^*$ in constant time per split or insertcompressed operation with the results from Section \ref{sec:dynamic} and \ref{sec:compression}. \ivor{Is this what we are trying to do or did I get it entirely wrong?}



\subsection{Adjusting Maarten's old algorithm.}

First of all we distinguish between four types of cells: Cells in the uncompressed component given by $R$ are denoted as $R$-cells. Cells in the uncompressed component of $S$ are denoted as $S$-cells. Roots of uncompressed components apart from $R$ in $A_1$ are denoted as $R'$-cells. And roots of uncompressed components apart from $S$ in $B_1$ are denoted as $S'$-cells. Note that the sets $R, S, R', S'$ do not have to overlap with one another in any organized way (see Figure \ref{fig:replacementexample}). The idea of the algorithm is that we use all the cells in $A_1$ to construct the $S$-cells. We then recurse on all the $S'$ cells to create each uncompressed component in $B_1$. \\

Just as in \cite{LM12}, we define the \textbf{frontier} $\mathcal{F}$ as the set of $S$-cells under $S$ which are leaves and intersect $R$. Observe that we can split $S$ until we find at most $3^d$ cells with a size $[|R|, 0.5|R|]$ in $\mathcal{F}$, denote this set as $L'$. 

\begin{itemize}
\item For every $C \in \mathcal{F}$, $AS(C)$ is the set of all \textbf{associated cells}.
$AS(C)$ are the smallest $R$-cells in $A_1$ such that have size at least $|C|$ \underline{and} intersect $C$, together with all the $R'$-cells that are contained in such an $R$ cell and intersect $C$. AS is stored with the leaves and compressed nodes first.
\item We call a cell $C \in \mathcal{F}$ \textbf{active} if $\exists R-cell \in AS(C)$ with $|R-cell| \in [|C|, 2|C|]$ or $\exists R'-cell \in AS(C)$ with $|R'-cell| \in [|C|/(3^d\alpha), |C|]$.
\item $L_1$ the set of all \textbf{active} cells in $\mathcal{F}$.
\item Note that at the start for each $C \in L'$, $AS(C) = R$ and $L = L'$.
\end{itemize}


\paragraph{Split operations on elements of $L$ can be performed in $\mathcal{O}((2d)^d)$ time.}
A split operations takes a cell $C \in \mathcal{F}$ and creates four new cells with four new associated lists. We can give each new child cell a new set $AS(C_{child})$ by copying $AS(C)$ and for each non leaf and non-compressed cell, removing that cell and adding the child cells that intersect $C_{child}$. Since we can skip the irrelevant leaves and compressed nodes in $\mathcal{O}(1)$ time, this takes $\mathcal{O}(2^d)$ time. \ivor{does it? really? cuz how many candidate cells do you need to check? not $(2^d)^m$?}

\subsubsection{The program loop.}

\paragraph{Iterating over $L$}

We simply split cells in $L$ until $L$ is empty. If $L$ is empty, there are no active cells so for each cell $C \in \mathcal{F}$. $AS(C)$ is filled with huge leaf squares and compressed nodes within more than $\log(\alpha)$ levels of $C$. Note that compressed cells are only stored in leaves so for each $C \in \mathcal{F}$, $|AS(C)| \le 3^d$. For each $C \in \mathcal{F}$ we construct $AS_2(C)$: the set of all points contained in $C$ together with all compressed roots in $AS(C)$. Clearly $|AS_2(C)| \le AS(C)$ since each point must be contained in a leaf cell in $AS(C)$. \\


\paragraph{Iterating over $L_2$.}
Given each $C \in \mathcal{F}$ and their set $AS_2(C)$ we need to store each point in $AS_2(C)$ with a compressed link. However, compressed links can only occur in leaf cells so we probably need to split all the $C \in \mathcal{F}$. We call a cell $C$ \textbf{postactive} if the bounding box that contains $AS_2(C)$ has a size larger than $|C|/(3^d\alpha)$ OR if $|AS_2(C)| > 1$. In other words: if there cannot exist a single compressed root that contains all the points. The list of all postactive cells is denoted as $L_2$. Observe that splitting a cell in $L_2$ allows us to create $2^d$ new cells in $\mathcal{O}(1)$ with a correct $As_2(C_{child})$ in $\mathcal{O}(1)$ time per child cell. We split all cells in $L_2$ until $L_2$ is empty. In that case, either each cell in $\mathcal{F}$ is a leaf which contains a single point or a leaf that should contain a single root of a compressed component. In the latter case, we recurse.

\subsubsection{Recursion on $C$}







==> Summary.tex <==
%\section{Summary}



\section{Extending the proof of Section \ref{sec:static} to work for $\mathbb{R}^d$.}
\label{sec:dimensionssum}

In this section, we prove that $T^*$ is smooth in every dimension $d$ if $T_1$ is an uncompressed quadtree.
Due to space restrictions, we only summarize the result here; the full details are defered to  Appendix \ref{sec:dimensions}.

In
Section \ref{sec:dynamic} we already elaborated on how we can dynamically maintain our extended quadtree $T^*$ in at most $\mathcal{O}((2d)^d)$ operations per split and merge on the true tree $T_1$. What remains to be proven is that the extended quadtree is indeed a smooth quadtree. We prove this by proving a generalized version of Theorem \ref{theorem:R2} in Section \ref{sec:static}:

%repeattheorem to make sure it has the same number every time it is stated
\begin{repeattheorem}{theorem:RD}
\label{theorem:RDsum}
Let $T_1$ be non-compressed quadtree over $\mathbb{R}^d$ which takes $\mathcal{O}(n)$ space. In the extended tree $T^*$ there cannot be two neighboring leaf cells which we will name $C_{d+1}$, $C_{d+2}$ with both brand $(d+1)$ such that $|C_{d+1}| \le \frac{1}{2^{d+1}}|C_{d+2}|$.
\end{repeattheorem}

The proof is similar to the proof in Section \ref{sec:R2}. If the two neighboring cells $C_{d+1}$ and $C_{d+2}$ want to exist in the plane then there must be a \textbf{chain} of $d$ cells ($C_d$ to $C_1$) with decreasing brand that forces the cells to exist. We show that it is impossible to embed this chain into the plane without either needing to split the largest cell or violating the \emph{Branding Principle} (Lemma \ref{lemma:brandingprinciple}). The difficulty of this proof is that there are many ways to embed such a chain of cells in $\mathbb{R}^d$. Moreover, if you want a cell $C_j$ in the chain to cause a contradiction with a neighboring cell you need to prove that the neighbor actually exists. We define an abstract virtual operator that can traverse the extended quadtree. With that operator and Lemma \ref{lemma:relation} in place we show that if you want to place $C_{d+2}$ to $C_1$ in the pane, then each time we must let $C_j$ neighbor $C_{j+1}$ in a unique dimension. If we use a dimension $\vec{y}$ twice we distinguish between two cases: 


The first case is that we use the same dimension and same direction. This case is equal to case 1 in Section \ref{sec:R2} and we show 
 that we must violate the \emph{Branding Principle}. 

%
The second case is that we use the same dimension and opposite direction and it corresponds with case 2 in Section \ref{sec:R2}. In this case we show that $C_{d+2}$ must have been split.

The result is that we need $(d+1)$ different dimensions to embed the chain but we have only $d$, a contradiction.

\section{Compressed quadtrees in $\mathbb{R}^d$.}
\label{sec:compressionsum}


The remainder of our work focuses on building smooth quadtrees that store a set of points and that are dynamic with respect to insertions and deletions of points from the set. If we want to build a dynamic quadtree over a point set of unbounded spread we need the quadtree to be compressed. We again want to define an extended quadtree $T^*$ that we can maintain with the operations in Section \ref{sec:dynamic}. 
In this section we extend our results to compressed quadtrees; the full details can be found in Appendix~\ref{sec:compression}.

Recall that in Definition \ref{def:t-star} We had $(d+1)$ different sets of cells where each set $T_j$ was defined as the minimal number of cells needed to balance the cells in $T_{j-1}$. We showed that if we have two uncompressed quadtrees $T_1$ and $T_1'$ which only differ by one split/merge operation that their extended quadtrees $T^*$ and $T'^*$ only differ in $\mathcal{O}((2d)^d)$ cells. However, if $T_1$ and $T_1'$ are uncompressed quadtrees and if we use Definition \ref{def:tree}, the reader can imagine that there are scenarios where their extended quadtrees $T^*$ and $T'^*$ differ in an arbitrarily large number of cells (see Appendix \ref{appendix:compression}). This is why instead we redefine our extended quadtree as the union of all extended quadtrees $A^*$ of all uncompressed components $A_1$ of $T_1$: $T^* := \cup_{\textit{Uncompressed components} A_1}A^*$. 
If we only demand that cells in uncompressed components count towards smoothness (the other cells are not stored anyway) then this extended quadtree is clearly smooth if Theorem \ref{theorem:RDsum} holds. However, Theorem \ref{theorem:RDsum} relies on Lemma \ref{lemma:relation} that says that cells that are \emph{family related} have a related brand and with this definition of $T^*$ we can place cells with an arbitrary high brand "on top" of other cells. We observe that the proof of Theorem \ref{theorem:RDsum} only uses paths that traverse $d^2$ levels of depth in the tree and we define additional operators that make sure that for each cell $C$, all ancestors within $d^2$ levels of  $C$ have a correct brand. The result is the following theorem:

\begin{repeattheorem}{theorem:changes}
\label{theorem:changes}
For each dynamic compressed quadtree $T_1$ over $\mathbb{R}^d$ we can maintain a smooth variant $T^*$ with at most:
\begin{itemize}
\item $\mathcal{O}((2d)^d)$ operations per split or merge on $T_1$.
\item $\mathcal{O}(\log(\alpha) d^2 (6d)^{d+1})$  operations per deletion or insertion of a compressed leaf.
\item $\mathcal{O}(d^2(6d)^d)$ time per upgrowing or downgrowing.
\end{itemize}
\end{repeattheorem}

\section{Alignment in Real RAM.}
\label{sec:alignmentsum}

Finally, we show that we can maintain non-aligned compressed quadtrees; the full details can be found in Appendix~\ref {sec:alignment}. 
In the previous section we 
were treating our compressed quadtree as if 
for  each compressed component $A_1$, the cell of its root $R$ was {\em aligned} with the cell of the leaf $C_a$ that stores its compressed link.
That is, the cell of  $R$ can be obtained by repeatedly subdividing the cell of $C_a$. 
However, finding an aligned cell for the root of a new uncompressed component when it is inserted is not supported in constant time in Real RAM model of computation. 
The reason is that the length of the compressed link, and thus the number of divisions necessary to compute the aligned root cell, may be arbitrary. 

Instead of computing the aligned root cell at the insertion of each new compressed component, we allow compressed nodes to be associated with any hypercube of an appropriate size that is contained in the cell of the compressed ancestor $C_a$.
For any compressed link in $T^*$, if the length of the link is at most $4\alpha$, 
then we must ensure that the corresponding uncompressed component is aligned with the parent cell of the link.  In~\cite{lss13} (full version), L\"{o}ffler \etal obtain this in amortized additional $O(1)$ time by  relocating the uncompressed component just before the decompression operation starts. We adjust their algorithm in three ways: (i) we make sure that their algorithm produces not a 2-smooth quadtree but our extended quadtree $T^*$. (ii) We de-amortize their algorithm with an adaption of a well-known de-amortization technique where you construct a correct copy of the unaligned uncompressed component. (iii) We extend the analysis in~\cite{lss13} so that their algorithm works in $\mathbb{R}^d$.  

\begin{repeattheorem}{thm:dd-const-alignment}
Let $P$ be a point set in $\mathbb{R}^d$ and $T_1$ be an $\alpha$-compressed quadtree over $P$ for a sufficiently big constant $\alpha$ with $\alpha > 2^{2^d}$ and 
$T^*$ be the extended variant of $T_1$ according to  Definition~\ref{definition:T-star-final}.  
The operations split and upgrowing on $T^*$ can be modified to 
maintain the alignment property 
for $T^*$. The modified operations require worst-case $O(32^d + d^2 \cdot (6d)^{d})$ time. % as the original operations.  
\end{repeattheorem}
%We elaborate on the application of our results in Appendix \ref{sec:applications}. 


